Fundamental Limitations in Performance and Interpretability of Common Planar Rigid-Body Contact Models

The ability to reason about and predict the outcome of contacts is paramount to the successful execution of many robot tasks. Analytical rigid-body contact models are used extensively in planning and control due to their computational efficiency and simplicity, yet despite their prevalence, little if any empirical comparison of these models has been made and it is unclear how well they approximate contact outcomes. In this paper, we first formulate a system identification approach for six commonly used contact models in the literature, and use the proposed method to find parameters for an experimental data-set of impacts. Next, we compare the models empirically, and establish a task specific upper bound on the performance of the models and the rigid-body contact model paradigm. We highlight the limitations of these models, salient failure modes, and the care that should be taken in parameter selection, which are ultimately difficult to give a physical interpretation.

==> referenc.tex <==
%%%%%%%%%%%%%%%%%%%%%%%% referenc.tex %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% sample references
% %
% Use this file as a template for your own input.
%
%%%%%%%%%%%%%%%%%%%%%%%% Springer-Verlag %%%%%%%%%%%%%%%%%%%%%%%%%%
%
% BibTeX users please use
% \bibliographystyle{}
% \bibliography{}
%
\biblstarthook{References may be \textit{cited} in the text either by number (preferred) or by author/year.\footnote{Make sure that all references from the list are cited in the text. Those not cited should be moved to a separate \textit{Further Reading} section or chapter.} The reference list should ideally be \textit{sorted} in alphabetical order -- even if reference numbers are used for the their citation in the text. If there are several works by the same author, the following order should be used: 
\begin{enumerate}
\item all works by the author alone, ordered chronologically by year of publication
\item all works by the author with a coauthor, ordered alphabetically by coauthor
\item all works by the author with several coauthors, ordered chronologically by year of publication.
\end{enumerate}
The \textit{styling} of references\footnote{Always use the standard abbreviation of a journal's name according to the ISSN \textit{List of Title Word Abbreviations}, see \url{http://www.issn.org/en/node/344}} depends on the subject of your book:
\begin{itemize}
\item The \textit{two} recommended styles for references in books on \textit{mathematical, physical, statistical and computer sciences} are depicted in ~\cite{science-contrib, science-online, science-mono, science-journal, science-DOI} and ~\cite{phys-online, phys-mono, phys-journal, phys-DOI, phys-contrib}.
\item Examples of the most commonly used reference style in books on \textit{Psychology, Social Sciences} are~\cite{psysoc-mono, psysoc-online,psysoc-journal, psysoc-contrib, psysoc-DOI}.
\item Examples for references in books on \textit{Humanities, Linguistics, Philosophy} are~\cite{humlinphil-journal, humlinphil-contrib, humlinphil-mono, humlinphil-online, humlinphil-DOI}.
\item Examples of the basic Springer style used in publications on a wide range of subjects such as \textit{Computer Science, Economics, Engineering, Geosciences, Life Sciences, Medicine, Biomedicine} are ~\cite{basic-contrib, basic-online, basic-journal, basic-DOI, basic-mono}. 
\end{itemize}
}

\begin{thebibliography}{99.}%
% and use \bibitem to create references.
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Contribution 
\bibitem{science-contrib} Broy, M.: Software engineering --- from auxiliary to key technologies. In: Broy, M., Dener, E. (eds.) Software Pioneers, pp. 10-13. Springer, Heidelberg (2002)
%
% Online Document
\bibitem{science-online} Dod, J.: Effective substances. In: The Dictionary of Substances and Their Effects. Royal Society of Chemistry (1999) Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{science-mono} Geddes, K.O., Czapor, S.R., Labahn, G.: Algorithms for Computer Algebra. Kluwer, Boston (1992) 
%
% Journal article
\bibitem{science-journal} Hamburger, C.: Quasimonotonicity, regularity and duality for nonlinear systems of partial differential equations. Ann. Mat. Pura. Appl. \textbf{169}, 321--354 (1995)
%
% Journal article by DOI
\bibitem{science-DOI} Slifka, M.K., Whitton, J.L.: Clinical implications of dysregulated cytokine production. J. Mol. Med. (2000) doi: 10.1007/s001090000086 
%
\bigskip

% Use the following (APS) syntax and markup for your references if 
% the subject of your book is from the field 
% "Mathematics, Physics, Statistics, Computer Science"
%
% Online Document
\bibitem{phys-online} J. Dod, in \textit{The Dictionary of Substances and Their Effects}, Royal Society of Chemistry. (Available via DIALOG, 1999), 
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Monograph
\bibitem{phys-mono} H. Ibach, H. L\"uth, \textit{Solid-State Physics}, 2nd edn. (Springer, New York, 1996), pp. 45-56 
%
% Journal article
\bibitem{phys-journal} S. Preuss, A. Demchuk Jr., M. Stuke, Appl. Phys. A \textbf{61}
%
% Journal article by DOI
\bibitem{phys-DOI} M.K. Slifka, J.L. Whitton, J. Mol. Med., doi: 10.1007/s001090000086
%
% Contribution 
\bibitem{phys-contrib} S.E. Smith, in \textit{Neuromuscular Junction}, ed. by E. Zaimis. Handbook of Experimental Pharmacology, vol 42 (Springer, Heidelberg, 1976), p. 593
%
\bigskip
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Psychology, Social Sciences"
%
%
% Monograph
\bibitem{psysoc-mono} Calfee, R.~C., \& Valencia, R.~R. (1991). \textit{APA guide to preparing manuscripts for journal publication.} Washington, DC: American Psychological Association.
%
% Online Document
\bibitem{psysoc-online} Dod, J. (1999). Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/Effective substances.} Cited 15 Jan 1999.
%
% Journal article
\bibitem{psysoc-journal} Harris, M., Karper, E., Stacks, G., Hoffman, D., DeNiro, R., Cruz, P., et al. (2001). Writing labs and the Hollywood connection. \textit{J Film} Writing, 44(3), 213--245.
%
% Contribution 
\bibitem{psysoc-contrib} O'Neil, J.~M., \& Egan, J. (1992). Men's and women's gender role journeys: Metaphor for healing, transition, and transformation. In B.~R. Wainrig (Ed.), \textit{Gender issues across the life cycle} (pp. 107--123). New York: Springer.
%
% Journal article by DOI
\bibitem{psysoc-DOI}Kreger, M., Brindis, C.D., Manuel, D.M., Sassoubre, L. (2007). Lessons learned in systems change initiatives: benchmarks and indicators. \textit{American Journal of Community Psychology}, doi: 10.1007/s10464-007-9108-14.
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Humanities, Linguistics, Philosophy"
%
\bigskip
%
% Journal article
\bibitem{humlinphil-journal} Alber John, Daniel C. O'Connell, and Sabine Kowal. 2002. Personal perspective in TV interviews. \textit{Pragmatics} 12:257--271
%
% Contribution 
\bibitem{humlinphil-contrib} Cameron, Deborah. 1997. Theoretical debates in feminist linguistics: Questions of sex and gender. In \textit{Gender and discourse}, ed. Ruth Wodak, 99--119. London: Sage Publications.
%
% Monograph
\bibitem{humlinphil-mono} Cameron, Deborah. 1985. \textit{Feminism and linguistic theory.} New York: St. Martin's Press.
%
% Online Document
\bibitem{humlinphil-online} Dod, Jake. 1999. Effective substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999
%
% Journal article by DOI
\bibitem{humlinphil-DOI} Suleiman, Camelia, Daniel C. O�Connell, and Sabine Kowal. 2002. `If you and I, if we, in this later day, lose that sacred fire...�': Perspective in political interviews. \textit{Journal of Psycholinguistic Research}. doi: 10.1023/A:1015592129296.
%
%
%
\bigskip
%
%
% Use the following syntax and markup for your references if 
% the subject of your book is from the field 
% "Computer Science, Economics, Engineering, Geosciences, Life Sciences"
%
%
% Contribution 
\bibitem{basic-contrib} Brown B, Aaron M (2001) The politics of nature. In: Smith J (ed) The rise of modern genomics, 3rd edn. Wiley, New York 
%
% Online Document
\bibitem{basic-online} Dod J (1999) Effective Substances. In: The dictionary of substances and their effects. Royal Society of Chemistry. Available via DIALOG. \\
\url{http://www.rsc.org/dose/title of subordinate document. Cited 15 Jan 1999}
%
% Journal article by DOI
\bibitem{basic-DOI} Slifka MK, Whitton JL (2000) Clinical implications of dysregulated cytokine production. J Mol Med, doi: 10.1007/s001090000086
%
% Journal article
\bibitem{basic-journal} Smith J, Jones M Jr, Houghton L et al (1999) Future of health insurance. N Engl J Med 965:325--329
%
% Monograph
\bibitem{basic-mono} South J, Blass B (2001) The future of modern genomics. Blackwell, London 
%
\end{thebibliography}


==> section_2/contact_model_details.tex <==
% \noindent \textbf{1) Anitescu-Potra (Newton).} 
%The numerical method developed in \cite{Anitescu:1997} and its close relative Stewart-Trinkle \cite{Stewart:1996} are both algebraic contact laws with a Newtonian restitution model relating the pre- and post-contact normal velocities. Anitescu-Potra generalizes the Glocker-Pfeiffer impact law~\cite{Chatterjee:1998,Glocker:1995}, when the latter is posed without tangential restitution. 

%\noindent \textbf{2) Anitescu-Potra (Poisson).}
%Anitescu and Potra also demonstrated the use of a Poissonian restitution in their model, this approach satisfies the kinetic energy constraint at the cost of solving two linear complementarity problems (LCPs)~\cite{Cottle:1992} per contact rather than one (though the solution to the second LCP is often trivial).

% \noindent \textbf{3) Drumwright-Shell.}
% Drumwright-Shell~\cite{Drumwright:2010b} is an algebraic, Poisson-type contact model that computes contact forces that maximize kinetic energy dissipation and does not incorporate the contact complementarity condition that arises from the equations for rigid contact between bodies at a single point.
% \begin{align}
    % \phi(\mathbf{q}) \ge 0, \quad f \ge 0, \quad f \cdot \phi(\mathbf{q}) = 0
% \end{align}
%% where $\phi(.)$ is the signed distance between two rigid bodies ($\phi < 0$ indicates interpenetration) at configuration $\mathbf{q}$, $f$ is the force applied along the contact normal (and $f \ge 0$ indicates that the force must be non-tensile), and $f \cdot \phi = 0$ is the complementarity condition.
%Drumwright-Shell drops this complementarity condition for computational efficiency, basing the omission on research by Chatterjee~\cite{Chatterjee:1999}) that showed that impacts need not respect complementarity. % Drumwright-Shell does not permit increases in kinetic energy for $0 \le \epsilon \le 1, \mu \ge 0$. This model was developed for 3D, but adapts naturally to 2D. 

% \noindent \textbf{4) Mirtich.}
% Mirtich's incremental collision model is a computational implementation~\cite{Mirtich:1996vt} of Stronge's work~\cite{Stronge:1990} relating physical work done in the compression and restitution phases of an contact. It does not permit increases in kinetic energy for $0 \le \epsilon \le 1,\ \mu \ge 0$. This is a fundamental 3D model that we adapted to 2D.

% \noindent \textbf{5) Wang-Mason.}
%The incremental Wang-Mason model relates the magnitude of the impulses in the compression and restitution phases of an impact~\cite{Wang:1992} (i.e., it is a Poisson-type~\cite{Poisson:1833} model). It is currently unknown whether the Wang-Mason model can predict increases in kinetic energy for $0 \le \epsilon \le 1, \mu \ge 0$. The Wang-Mason model is a 2D model.
%

% \noindent \textbf{6) Whittaker.}
%The Whittaker model is an algebraic model that requires solution to a nonlinear system of equations. It can predict arbitrarily large kinetic energy increases for $0 \le \epsilon \le 1, \mu \ge 0$. Both 2D~\cite{Whittaker:1944} and 3D versions~\cite{Kane:1985} have been studied.
%

%\noindent \textbf{7) Best Post Hoc.} \label{sec:best-model}
%This fictitious model selects the best performing model for each trial of the experiment after the fact, characterizing the best possible performance over the data-set for the analytical models studied in this paper. This model establishes an upper-bound on the predictive performance for the models \emph{under the assumption of state-independent coefficients of friction and restitution}.
% EDNOTE: I think you should elaborate on this thought a little (perhaps one more sentence). % EDNOTE: An interesting thing that we could note about this model is how frequently the Newtonian model is used in simulations by virtue of the popularity of the AP/ST model % NFNOTE: Good idea, I don't have the statistics now so we can revise this later.

% SZNOTE: This is the entire parameter-space of the model. This should be broken into 2 sentences.: --Replacing the current sentence: "The model can predict arbitrarily large kinetic energy increases." --And then at the top of the section where you declare mu and epsilon: "\epsilon is defined within the closed interval $0 \le \epsilon \le 1$; \mu is in the open interval $\mu \ge 0$."

==> section_5/figure_convex_error.tex <==
\begin{figure}[h]
  \centering
  \subfloat[Example 1.]
  {\includegraphics[width=0.45\textwidth]{section_5/figures/model_convex_error_spin_1.pdf}} ~
  \subfloat[Example 2.]
  {\includegraphics[width=0.45\textwidth]{section_5/figures/model_convex_error_spin_2.pdf}}
  \caption{Two example of cases where the measured impulse lies outside the convex set of predictions made by the model due to ``spin-reversal".}
  \label{fig:convex_error}
\end{figure}

==> section_5/figure_gpr.tex <==
\begin{figure}[h]
    \centering
    \subfloat[Number of data:  85 Drops.]
    {\includegraphics[width=0.45\textwidth]{section_5/figures/model_gp_norm_3.pdf}}~ 
    \subfloat[Number of data: 170 Drops.]
    {\includegraphics[width=0.45\textwidth]{section_5/figures/model_gp_norm_2.pdf}}

    \subfloat[Number of data: 450 Drops.]
    {\includegraphics[width=0.45\textwidth]{section_5/figures/model_gp_norm_1.pdf}}~
    \subfloat[Number of data: 1100 Drops.]
    {\includegraphics[width=0.45\textwidth]{section_5/figures/model_gp_norm_4.pdf}}
    \caption{Data-driven contact models: the Gaussian Process regression results.}  
  \label{fig:gpr}
\end{figure}

 


==> section_5/figures_best_average.tex <==
% Error norms average best

\begin{figure}[h]
  \centering
  \subfloat[Estimated PDF of the 2 norm error in impulse.]
  {\includegraphics[width=0.45\textwidth]{section_5/figures/model_momentum_norm.pdf}} ~
  \subfloat[Estimated PDF of the 2 norm error in velocity of the center of mass.]
  {\includegraphics[width=0.45\textwidth]{section_5/figures/model_velocity_norm.pdf}}
  \caption{Estimated partial density functions (PDFs) of the $\ell_2$-norm error in impulse (predicted versus inferred from data) and velocity of the center of mass (predicted versus measured).}
  \label{fig:norm}
\end{figure}
